HAT-P-50b, HAT-P-51b, HAT-P-52b, and HAT-P-53b: Three Transiting Hot Jupiters and a Transiting Hot Saturn From the HATNet Survey

We report the discovery and characterization of four transiting exoplanets by the HATNet survey. The planet HAT-P-50b has a mass of 1.35 M_J and a radius of 1.29 R_J, and orbits a bright (V = 11.8 mag) M = 1.27 M_sun, R = 1.70 R_sun star every P = 3.1220 days. The planet HAT-P-51b has a mass of 0.31 M_J and a radius of 1.29 R_J, and orbits a V = 13.4 mag, M = 0.98 M_sun, R = 1.04 R_sun star with a period of P = 4.2180 days. The planet HAT-P-52b has a mass of 0.82 M_J and a radius of 1.01 R_J, and orbits a V = 14.1 mag, M = 0.89 M_sun, R = 0.89 R_sun star with a period of P = 2.7536 days. The planet HAT-P-53b has a mass of 1.48 M_J and a radius of 1.32 R_J, and orbits a V = 13.7 mag, M = 1.09 M_sun, R = 1.21 R_sun star with a period of P = 1.9616 days. All four planets are consistent with having circular orbits and have masses and radii measured to better than 10% precision. The low stellar jitter and favorable R_P/R_star ratio for HAT-P-51 make it a promising target for measuring the Rossiter-McLaughlin effect for a Saturn-mass planet.

==> HTR165-010_rvtable.tex <==
$ 1877.91488 $ & $   217.41 $ & $     4.13 $ & $     3.37 $ & $     8.66 $ & $    0.1820 $ & $   0.708 $ & HIRES \\
$ 1879.81971 $ & $   220.06 $ & $     3.91 $ & $    -8.64 $ & $     5.38 $ & $    0.1710 $ & $   0.679 $ & HIRES \\
$ 1879.83898 $ & \nodata      & \nodata      & $    -6.30 $ & $     5.05 $ & $    0.1700 $ & $   0.689 $ & HIRES \\
$ 1880.95723 $ & $  -228.59 $ & $     3.82 $ & $     4.64 $ & $     4.22 $ & $    0.1740 $ & $   0.259 $ & HIRES \\
$ 1944.84748 $ & $   187.44 $ & $     5.04 $ & $    11.55 $ & $     4.67 $ & $    0.1010 $ & $   0.829 $ & HIRES \\
$ 1960.79667 $ & $    43.84 $ & $     4.68 $ & $   -10.07 $ & $    13.55 $ & $    0.1430 $ & $   0.959 $ & HIRES \\
$ 1972.75173 $ & $   -68.38 $ & $     4.23 $ & $   -14.42 $ & $     7.85 $ & $    0.1570 $ & $   0.054 $ & HIRES \\


==> HTR210-001_rvtable.tex <==
$ 1853.80027 $ & $   -42.75 $ & $     2.53 $ & $   -16.75 $ & $     5.54 $ & $    0.1550 $ & $   0.317 $ & HIRES \\
$ 1853.81798 $ & \nodata      & \nodata      & $    -2.36 $ & $     6.06 $ & $    0.1300 $ & $   0.322 $ & HIRES \\
$ 1879.85898 $ & \nodata      & \nodata      & $    10.56 $ & $     6.81 $ & $    0.1630 $ & $   0.495 $ & HIRES \\
$ 1879.87608 $ & $     7.25 $ & $     2.68 $ & $     8.32 $ & $     6.08 $ & $    0.1570 $ & $   0.499 $ & HIRES \\
$ 1880.97599 $ & $    42.01 $ & $     2.48 $ & $     9.54 $ & $     5.32 $ & $    0.0769 $ & $   0.760 $ & HIRES \\
$ 1903.95906 $ & $   -35.87 $ & $     2.63 $ & $   -42.11 $ & $    21.39 $ & $    0.1550 $ & $   0.209 $ & HIRES \\
$ 1944.73569 $ & $    24.93 $ & $     2.55 $ & $    -9.88 $ & $     7.15 $ & $    0.1170 $ & $   0.876 $ & HIRES \\
$ 1960.81411 $ & $    31.81 $ & $     3.23 $ & $     5.14 $ & $     7.02 $ & $    0.1600 $ & $   0.688 $ & HIRES \\
$ 1964.71582 $ & $    44.69 $ & $    13.17 $ & $    -0.33 $ & $    26.24 $ & \nodata      & $   0.613 $ & HDS \\
$ 1964.72359 $ & $    27.51 $ & $    11.37 $ & $   -23.77 $ & $    23.80 $ & \nodata      & $   0.615 $ & HDS \\
$ 1964.73475 $ & $    21.63 $ & $    11.55 $ & $     7.03 $ & $    29.96 $ & \nodata      & $   0.617 $ & HDS \\
$ 1964.74946 $ & $    25.14 $ & $     9.83 $ & $     3.26 $ & $    34.15 $ & \nodata      & $   0.621 $ & HDS \\
$ 1964.76417 $ & $    33.95 $ & $     9.59 $ & $     0.65 $ & $    35.27 $ & \nodata      & $   0.624 $ & HDS \\
$ 1965.71533 $ & $    32.14 $ & $    15.07 $ & $    -2.89 $ & $    24.12 $ & \nodata      & $   0.850 $ & HDS \\
$ 1965.73005 $ & $    29.21 $ & $    12.47 $ & $     9.32 $ & $    36.71 $ & \nodata      & $   0.853 $ & HDS \\
$ 1965.74477 $ & $    33.24 $ & $    11.95 $ & $   -14.30 $ & $    27.64 $ & \nodata      & $   0.857 $ & HDS \\
$ 1965.75948 $ & $    34.67 $ & $    14.11 $ & $   -16.82 $ & $    27.55 $ & \nodata      & $   0.860 $ & HDS \\
$ 1965.77418 $ & $    13.59 $ & $    12.75 $ & $    21.67 $ & $    22.10 $ & \nodata      & $   0.864 $ & HDS \\
$ 1965.78890 $ & $    15.87 $ & $    21.41 $ & $    23.88 $ & $    25.83 $ & \nodata      & $   0.866 $ & HDS \\
$ 1966.72018 $ & \nodata      & \nodata      & $    -4.21 $ & $    31.52 $ & \nodata      & $   0.088 $ & HDS \\
$ 1966.73489 $ & \nodata      & \nodata      & $     9.59 $ & $    32.96 $ & \nodata      & $   0.092 $ & HDS \\
$ 1966.74959 $ & \nodata      & \nodata      & $     4.25 $ & $    32.50 $ & \nodata      & $   0.095 $ & HDS \\
$ 1966.76429 $ & \nodata      & \nodata      & $     5.05 $ & $    34.50 $ & \nodata      & $   0.099 $ & HDS \\
$ 1966.77907 $ & $   -12.89 $ & $    12.16 $ & $    -0.33 $ & $    34.37 $ & \nodata      & $   0.102 $ & HDS \\
$ 1966.79377 $ & $   -33.08 $ & $    11.65 $ & $    27.17 $ & $    29.63 $ & \nodata      & $   0.106 $ & HDS \\
$ 1966.80848 $ & $   -13.58 $ & $    15.24 $ & $     5.11 $ & $    13.87 $ & \nodata      & $   0.109 $ & HDS \\
$ 1967.72003 $ & $   -24.46 $ & $    14.33 $ & $    -2.79 $ & $    22.98 $ & \nodata      & $   0.325 $ & HDS \\
$ 1967.73475 $ & $   -48.37 $ & $    13.90 $ & $   -12.59 $ & $    23.40 $ & \nodata      & $   0.329 $ & HDS \\
$ 1967.74946 $ & $   -42.32 $ & $    13.39 $ & $   -11.16 $ & $    21.89 $ & \nodata      & $   0.332 $ & HDS \\
$ 1967.76417 $ & $   -34.03 $ & $    12.75 $ & $     0.39 $ & $    20.57 $ & \nodata      & $   0.336 $ & HDS \\
$ 1967.77888 $ & $   -28.16 $ & $    13.62 $ & $     3.97 $ & $    17.43 $ & \nodata      & $   0.339 $ & HDS \\
$ 1967.79359 $ & $   -28.23 $ & $    14.33 $ & $   -32.17 $ & $    31.51 $ & \nodata      & $   0.343 $ & HDS \\


==> HTR212-005_rvtable.tex <==
$ 1611.81789 $ & $   134.02 $ & $     4.23 $ & $    17.97 $ & $    81.51 $ & $    0.2500 $ & $   0.738 $ & HIRES \\
$ 1853.86184 $ & $    90.96 $ & $     3.67 $ & $    -6.05 $ & $    13.12 $ & $    0.1870 $ & $   0.639 $ & HIRES \\
$ 1853.88098 $ & \nodata      & \nodata      & $    67.06 $ & $    32.55 $ & $    0.1230 $ & $   0.646 $ & HIRES \\
$ 1879.90065 $ & $   -62.91 $ & $     4.21 $ & $   -11.44 $ & $    32.23 $ & $    0.1220 $ & $   0.095 $ & HIRES \\
$ 1880.99970 $ & $     1.46 $ & $     3.24 $ & $    10.18 $ & $    16.84 $ & $    0.1500 $ & $   0.494 $ & HIRES \\
$ 1882.08871 $ & $    76.62 $ & $     7.72 $ & $   -77.06 $ & $    46.76 $ & $    0.4450 $ & $   0.890 $ & HIRES \\
$ 1972.84557 $ & $   102.30 $ & $     4.25 $ & \nodata      & \nodata      & \nodata      & $   0.849 $ & HIRES \\
$ 2139.06062 $ & $  -134.45 $ & $     3.86 $ & $    -0.66 $ & $    15.61 $ & $    0.1360 $ & $   0.212 $ & HIRES \\


==> HTR316-006_rvtable.tex <==
$ 1903.95158 $ & $   169.24 $ & $    31.82 $ & \nodata      & \nodata      & \nodata      & $   0.656 $ & TRES \\
$ 1911.98432 $ & $  -149.26 $ & $    31.82 $ & \nodata      & \nodata      & \nodata      & $   0.229 $ & TRES \\
$ 1941.89144 $ & $    -5.12 $ & $    65.07 $ & \nodata      & \nodata      & \nodata      & $   0.808 $ & TRES \\
$ 1957.72714 $ & $    81.84 $ & $    63.24 $ & \nodata      & \nodata      & \nodata      & $   0.881 $ & TRES \\
$ 1958.68285 $ & $   -19.27 $ & $    59.81 $ & \nodata      & \nodata      & \nodata      & $   0.187 $ & TRES \\
$ 1960.70621 $ & $   -26.06 $ & $    73.39 $ & \nodata      & \nodata      & \nodata      & $   0.835 $ & TRES \\
$ 1964.90560 $ & $  -161.79 $ & $    16.35 $ & $   -44.94 $ & $    22.34 $ & \nodata      & $   0.180 $ & HDS \\
$ 1964.91336 $ & $  -158.48 $ & $    15.07 $ & $   -40.90 $ & $    21.84 $ & \nodata      & $   0.182 $ & HDS \\
$ 1964.92112 $ & $  -164.86 $ & $    14.23 $ & $   -54.18 $ & $    20.02 $ & \nodata      & $   0.185 $ & HDS \\
$ 1964.93269 $ & \nodata      & \nodata      & $   -62.87 $ & $    21.17 $ & \nodata      & $   0.189 $ & HDS \\
$ 1964.94740 $ & \nodata      & \nodata      & $   -62.65 $ & $    21.82 $ & \nodata      & $   0.193 $ & HDS \\
$ 1964.96211 $ & \nodata      & \nodata      & $   -61.14 $ & $    22.32 $ & \nodata      & $   0.198 $ & HDS \\
$ 1965.06347 $ & $  -184.08 $ & $    15.46 $ & $  -110.01 $ & $    24.62 $ & \nodata      & $   0.231 $ & HDS \\
$ 1965.07123 $ & $  -196.36 $ & $    14.93 $ & $  -153.60 $ & $    27.34 $ & \nodata      & $   0.233 $ & HDS \\
$ 1966.86139 $ & $   143.00 $ & $    14.72 $ & $   -32.02 $ & $    20.00 $ & \nodata      & $   0.807 $ & HDS \\
$ 1966.87609 $ & $   137.51 $ & $    13.33 $ & $   -19.54 $ & $    19.70 $ & \nodata      & $   0.811 $ & HDS \\
$ 1967.86542 $ & $   -96.04 $ & $    21.28 $ & $    -7.35 $ & $    21.69 $ & \nodata      & $   0.128 $ & HDS \\
$ 1967.87318 $ & $   -93.64 $ & $    18.64 $ & $   -15.27 $ & $    20.80 $ & \nodata      & $   0.131 $ & HDS \\
$ 1967.88093 $ & $   -87.90 $ & $    16.20 $ & $     0.26 $ & $    18.99 $ & \nodata      & $   0.133 $ & HDS \\
$ 1967.88867 $ & $  -108.44 $ & $    17.37 $ & $    -9.93 $ & $    20.59 $ & \nodata      & $   0.135 $ & HDS \\
$ 2000.39479 $ & $    78.60 $ & $    23.25 $ & \nodata      & \nodata      & \nodata      & $   0.547 $ & FIES \\
$ 2001.40519 $ & $   121.33 $ & $    23.25 $ & \nodata      & \nodata      & \nodata      & $   0.871 $ & FIES \\
$ 2002.47018 $ & $  -191.77 $ & $    30.26 $ & \nodata      & \nodata      & \nodata      & $   0.212 $ & FIES \\
$ 2003.40044 $ & $     4.13 $ & $    54.05 $ & \nodata      & \nodata      & \nodata      & $   0.510 $ & FIES \\
$ 2004.38851 $ & $   120.16 $ & $    31.15 $ & \nodata      & \nodata      & \nodata      & $   0.827 $ & FIES \\
$ 2191.13792 $ & $   121.23 $ & $    22.53 $ & $    45.30 $ & $    19.61 $ & \nodata      & $   0.644 $ & HDS \\
$ 2191.14223 $ & $   129.48 $ & $    26.61 $ & $   129.85 $ & $    21.78 $ & \nodata      & $   0.645 $ & HDS \\
$ 2191.14652 $ & $   184.86 $ & $    29.91 $ & $   496.30 $ & $    30.08 $ & \nodata      & $   0.647 $ & HDS \\
$ 2192.12442 $ & $    48.71 $ & $    17.29 $ & $     7.33 $ & $    16.97 $ & \nodata      & $   0.960 $ & HDS \\
$ 2192.12871 $ & $    45.28 $ & $    23.29 $ & $    -3.33 $ & $    20.31 $ & \nodata      & $   0.961 $ & HDS \\
$ 2192.13300 $ & $    28.57 $ & $    21.63 $ & $     9.00 $ & $    17.56 $ & \nodata      & $   0.963 $ & HDS \\
$ 2193.11572 $ & $  -151.84 $ & $    16.13 $ & $    -7.12 $ & $    19.16 $ & \nodata      & $   0.277 $ & HDS \\
$ 2193.12002 $ & $  -121.63 $ & $    23.24 $ & $    -5.25 $ & $    17.21 $ & \nodata      & $   0.279 $ & HDS \\
$ 2193.12433 $ & $  -127.80 $ & $    20.99 $ & $     2.08 $ & $    16.32 $ & \nodata      & $   0.280 $ & HDS \\


==> newcommand_spec_multi_template.tex <==
%% GB's various newcommands for making editing easy for this specific paper

% This is the template version to be used for planets announced in a
% multi-planet paper. This file should be filled in separately for
% each planet in the paper. You should also find/replace the term
% xxxxx below with a unique identifier for each planet (e.g. xxxxA for
% the first one).  A version of this file should be saved with a
% unique name in the document directory for each planet, and all files
% should be processed into the newcommand_spec_multi.tex file using
% the scr/makenewcommand_spec_multi.sh script. This is done to allow
% you to reference planet information using commands like \hatcur{14}
% rather than \hatcurxxxxA. The newcommand_spec_multi.tex file so
% generated should not need to be edited or regenerated if changes are
% made to any of the planets parameters. Any changes should be made to
% the planet's own newcommand_spec.tex file.

% -------- Aliases specific to this paper/planet which should be edited -------

% The name of the host star and/or the planet:
\newcommand{\hatcurxxxxx}{HAT-P-14}
\newcommand{\hatcurbxxxxx}{HAT-P-14b}
\newcommand{\hatcurcxxxxx}{HAT-P-14c}

% The number used to index this system in the paper
\newcommand{\hatcurplanetnumxxxxx}{14}

%\newcommand{\hatcurCCraxxxxx}{\ensuremath{08^{\mathrm h}39^{\mathrm m}31.82^{\mathrm s}}}  % right ascension
%\newcommand{\hatcurCCdecxxxxx}{\ensuremath{+47^{\mathrm d}21^{\mathrm m}07.4^{\mathrm s}}} % declination

\newcommand{\hatcurRVgammaabsxxxxx}{\hatcurDSgamma{\hatcurplanetnumxxxxx}}                           % Absolute Gamma velocity

\newcommand{\hatcurRVgammarelxxxxx}{\hatcurRVgamma{\hatcurplanetnumxxxxx}}                           % Relative Gamma velocity. Typically that of the Keck RVs.

\newcommand{\hatcurCCtassvixxxxx}{\ensuremath{0.527\pm0.12}}                  % TASS V-I

\newcommand{\hatcurSMEversionxxxxx}{ii}                                       % Final SME version:i or ii?

% Isochrones used for this planet.
\newcommand{\hatcurisoshortxxxxx}{YY}
%\newcommand{\hatcurisoshortxxxxx}{Baraffe}
\newcommand{\hatcurisofullxxxxx}{Yonsei-Yale (YY)}
%\newcommand{\hatcurisofullxxxxx}{Baraffe}
\newcommand{\hatcurisocitexxxxx}{yi:2001}
%\newcommand{\hatcurisocitexxxxx}{baraffe:1998}

% Luminosity indicator used for this planet.
\newcommand{\hatcurlumindxxxxx}{\arstar}
%\newcommand{\hatcurlumindxxxxx}{Hip}s

% JHK filter type for the isochrone set used for this planet.
\newcommand{\hatcurjhkfilsetxxxxx}{ESO}
%\newcommand{\hatcurjhkfilsetxxxxx}{BB}
%\newcommand{\hatcurjhkfilsetxxxxx}{CIT}

% --------------------------------------------------------------------------
% The aliases below should not need editing, other than replaceing xxxxxx
% to whatever string.
% 
\newcommand{\hatcurSMEteffxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEiteff{\hatcurplanetnumxxxxx}}{\hatcurSMEiiteff{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEzfehxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEizfeh{\hatcurplanetnumxxxxx}}{\hatcurSMEiizfeh{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEzfehshortxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEizfehshort{\hatcurplanetnumxxxxx}}{\hatcurSMEiizfehshort{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEloggxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEilogg{\hatcurplanetnumxxxxx}}{\hatcurSMEiilogg{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvsinxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivsin{\hatcurplanetnumxxxxx}}{\hatcurSMEiivsin{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvmacxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivmac{\hatcurplanetnumxxxxx}}{\hatcurSMEiivmac{\hatcurplanetnumxxxxx}}}
\newcommand{\hatcurSMEvmicxxxxx}{\ifthenelse{\equal{\hatcurSMEversionxxxxx}{i}}{\hatcurSMEivmic{\hatcurplanetnumxxxxx}}{\hatcurSMEiivmic{\hatcurplanetnumxxxxx}}}

